Morfessor EM+Prune: Improved Subword Segmentation with Expectation Maximization and Pruning

Data-driven segmentation of words into subword units has been used in various natural language processing applications such as automatic speech recognition and statistical machine translation for almost 20 years. Recently it has became more widely adopted, as models based on deep neural networks often benefit from subword units even for morphologically simpler languages. In this paper, we discuss and compare training algorithms for a unigram subword model, based on the Expectation Maximization algorithm and lexicon pruning. Using English, Finnish, North Sami, and Turkish data sets, we show that this approach is able to find better solutions to the optimization problem defined by the Morfessor Baseline model than its original recursive training algorithm. The improved optimization also leads to higher morphological segmentation accuracy when compared to a linguistic gold standard. We publish implementations of the new algorithms in the widely-used Morfessor software package.

==> table_analysis_fin.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llrrrr|rrrrrr}
\toprule
                                  &                 & \multicolumn{4}{c}{Over-segmentation}  & \multicolumn{6}{c}{Under-segmentation} \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-12}
                          Model   & \vh{Forcesplit} & \vh{STM}  & \vh{SUF}  & \vh{UNKNOWN}  & \vh{\bf{PRE/TOT}} & \vh{STM-SUF} & \vh{STM-STM}   & \vh{SUF-SUF}   & \vh{SUF-STM}   & \vh{UNKNOWN}   & \vh{\bf{REC/TOT}} \\
 %                        Model                       Over.STM    Over.SUF    Over.UNKNOWN    Over.Total          Under.STM-SUF    Under.STM-STM    Under.SUF-SUF    Under.SUF-STM    Under.UNKNOWN    Under.Total
 \midrule
 Characters                           &             &     65.23  &       13.80  &         0.57  &      19.73  &                    0.00  &            0.00  &                0.00  &              0.00  &          0.00  &      100.00  \\
 Words                                &             &      0.00  &        0.00  &         0.00  &     100.00  &                   49.19  &           17.16  &               21.76  &              4.84  &          0.58  &        4.09  \\
 \midrule
 Morfessor Baseline                   &             &     34.75  &        2.82  &         0.38  &      62.02  &                   24.57  &       \bb  0.86  &               16.31  &        \bb   0.15  &          0.20  &       57.63  \\
 Morfessor Baseline                   & \checkmark  &     34.50  &        2.80  &         0.36  &      62.30  &              \bb  24.33  &            0.88  &               16.31  &        \bb   0.15  &     \bb  0.10  &   \bb 58.19  \\
 SentencePiece 13k                    &             &     35.11  &        3.71  &         0.41  &      60.69  &                   25.96  &            1.45  &               16.18  &              0.35  &          0.16  &       55.81  \\
 \midrule
\bb EM+P     MDL                      & \checkmark  &     29.22  &        2.18  & \bb     0.22  &      68.34  &                   24.60  &            0.91  &               15.94  &              0.29  &     \bb  0.10  &       58.11  \\
 EM+P     MDL                         &             &     29.34  &        2.20  &         0.26  &      68.18  &                   24.68  &            0.90  &               15.95  &              0.29  &          0.19  &       57.60  \\
%EM+P     (ca spm 13k)                &             &     33.14  &        2.81  &         0.38  &      63.61  &                   27.62  &            1.25  &               15.73  &              0.35  &          0.20  &       54.44  \\
 EM+P     MDL lateen                  & \checkmark  &     28.84  &        2.06  & \bb     0.22  & \bb  68.86  &                   25.78  &            0.93  &               16.39  &              0.37  &          0.12  &       56.36  \\
%EM+P     MDL lateen                  &             &     28.96  &        2.05  &         0.24  &      68.72  &                   25.75  &            0.93  &               16.35  &              0.36  &          0.19  &       56.02  \\
%EM+P     MDL      noexp$\Psi$        &             &     29.22  &        2.19  &         0.26  &      68.30  &                   24.90  &            0.91  &               15.79  &              0.29  &          0.19  &       57.55  \\
 EM+P     MDL      noexp$\Psi$        & \checkmark  &     29.16  &        2.18  & \bb     0.22  &      68.40  &                   24.85  &            0.92  &               15.90  &              0.29  &     \bb  0.10  &       57.89  \\
%EM+P     MDL      nofreqdistr        &             &     29.19  &        2.14  &         0.25  &      68.38  &                   24.83  &            0.92  &               15.84  &              0.30  &          0.19  &       57.55  \\
 EM+P     MDL      nofreqdistr        & \checkmark  &     29.07  & \bb    2.02  & \bb     0.22  &      68.66  &                   24.76  &            0.94  &               15.86  &              0.30  &          0.11  &       57.98  \\
%EM+P     MDL      nofreqdistr nored  & \checkmark  &     28.74  &        1.99  &         0.21  &      69.03  &                   24.75  &            0.95  &               15.71  &              0.30  &          0.11  &       58.13  \\
 EM+P     MDL      nored              &             &     29.01  &        2.11  &         0.26  &      68.59  &                   24.77  &            0.90  &               15.74  &              0.26  &          0.20  &       57.74  \\
 EM+P     MDL      nored noexp$\Psi$  &             & \bb 28.77  &        2.08  &         0.26  &      68.85  &                   24.70  &            0.92  &          \bb  15.68  &              0.29  &          0.20  &       57.83  \\
 EM+P     auto     lateen 13k         & \checkmark  &     29.30  &        2.07  & \bb     0.22  &      68.38  &                   25.22  &            0.89  &               16.32  &              0.36  &          0.12  &       57.04  \\

\bottomrule
\end{tabular}}
\caption{\fixme{Error analysis for Finnish. Over-segmentation and under-segmentation errors reduce
precision and recall, respectively. $\alpha=0.02$}
\label{tab:error:fin}}
\end{table*}


==> table_analysis_sme.tex <==
\begin{table*}[t]
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{llrrr|rrrrr}
\toprule
                                  &                 & \multicolumn{3}{c}{Over-segmentation}  & \multicolumn{5}{c}{Under-segmentation} \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-10}
                          Model   & \vh{Forcesplit} & \vh{STM}  & \vh{SUF}  & \vh{\bf{PRE/TOT}} & \vh{STM-SUF} & \vh{STM-STM}   & \vh{SUF-SUF}   & \vh{SUF-STM}   & \vh{\bf{REC/TOT}} \\
 %                        Model                       Over.STM    Over.SUF    Over.Total          Under.STM-SUF    Under.STM-STM    Under.SUF-SUF    Under.SUF-STM    Under.Total
 \midrule
 Characters                           &             &     81.44  &        6.80  &      11.76  &                    0.00  &            0.00  &                0.00  &              0.00  &      100.00    \\
 Words                                &             &      0.00  &        0.00  &     100.00  &                   52.92  &           13.15  &                4.43  &              0.61  &       28.64    \\
 \midrule
 Morfessor Baseline                   &             &     23.27  &  \bb   3.02  &      73.71  &                   33.16  &      \bb   2.22  &                3.40  &        \bb   0.10  &       60.99    \\
 Morfessor Baseline                   & \checkmark  &     22.91  &        3.33  & \bb  73.76  &                   33.07  &      \bb   2.22  &                3.47  &        \bb   0.10  &       61.14    \\
 SentencePiece 64k                    &             &     30.10  &        4.52  &      65.38  &                   31.35  &            3.96  &          \bb   3.09  &              0.20  &       61.40    \\
 \midrule
\bb EM+P     MDL                      & \checkmark  &     23.09  &        4.41  &      72.50  &                   30.60  &            3.10  &                3.23  &              0.17  &       62.90    \\
 EM+P     MDL                         &             &     23.35  &        4.41  &      72.25  &                   30.48  &            3.10  &                3.23  &              0.17  &       62.84    \\
%EM+P     MDL lateen                  & \checkmark  &     23.65  &        4.41  &      71.94  &                   33.36  &            2.97  &                3.30  &              0.17  &       60.20    \\
 EM+P     MDL lateen                  &             &     23.63  &        4.39  &      71.98  &                   33.28  &            2.97  &                3.30  &              0.17  &       60.15    \\
%EM+P     MDL lateen noexp$\Psi$      &             &     22.23  &        4.03  &      73.74  &                   33.64  &            3.16  &                3.23  &              0.17  &       59.67    \\
%EM+P     MDL lateen nofreqdistr      &             &     22.18  &        4.22  &      73.60  &                   33.99  &            3.16  &                3.17  &              0.17  &       59.32    \\
%EM+P     MDL lateen nofreqdistr      & \checkmark  &     21.83  &        4.34  &      73.83  &                   33.87  &            3.22  &                3.23  &              0.17  &       59.51    \\
 EM+P     MDL      noexp$\Psi$        &             &     24.86  &        4.42  &      70.72  &              \bb  30.35  &            2.97  &                3.34  &              0.17  &   \bb 63.04    \\
%EM+P     MDL      nofreqdistr        & \checkmark  &     22.18  &        4.34  &      73.47  &                   31.79  &            3.10  &                3.23  &              0.17  &       61.70    \\
 EM+P     MDL      nofreqdistr        &             & \bb 22.16  &        4.47  &      73.37  &                   31.98  &            3.10  &                3.23  &              0.17  &       61.39    \\

\bottomrule
\end{tabular}%}
\caption{\fixme{Error analysis for North Sámi. Over-segmentation and under-segmentation errors reduce
precision and recall, respectively. $\alpha=1.0$}
\label{tab:error:sme}}
\end{table*}


==> table_train_variants.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
                    & \multicolumn{3}{c}{Pruning criterion} \\
\cmidrule{2-4}
                    & MDL           & Autotune      & Lexicon       \\
\midrule
Hyper-parameter     & $\alpha$      & $|\lexicon|$  & $|\lexicon|$  \\
\midrule
%Prior       \\
Full prior          & \checkmark    & \checkmark    & (\checkmark)  \\
Without Bayesian EM & \checkmark    & \checkmark    & (\checkmark)  \\
Omitting frequency  & \checkmark    & \checkmark    & (\checkmark)  \\
Omitting prior      & --            & --            & \checkmark    \\
\bottomrule
\end{tabular}}
\caption{\fixme{Training variants.}
\label{tab:trainvariants}}
\end{table}

